(Towards) Scalable Reliable Automated Evaluation with Large Language Models

Evaluating the quality and relevance of textual outputs from Large Language Models (LLMs) remains challenging and resource-intensive. Existing automated metrics often fail to capture the complexity and variability inherent in LLM-generated outputs. Moreover, these metrics typically rely on explicit reference standards, limiting their use mostly to domains with objective benchmarks. This work introduces a novel evaluation framework designed to approximate expert-level assessments of LLM-generated content. The proposed method employs pairwise comparisons of outputs by multiple LLMs, reducing biases from individual models. An Elo rating system is used to generate stable and interpretable rankings. Adjustable agreement thresholds, from full unanimity to majority voting, allow flexible control over evaluation confidence and coverage. The method's effectiveness is demonstrated through evaluating competency profiles extracted from scientific abstracts. Preliminary results show that automatically derived rankings correlate well with expert judgments, significantly reducing the need for extensive human intervention. By offering a scalable, consistent, and domain-agnostic evaluation layer, the framework supports more efficient and reliable quality assessments of LLM outputs across diverse applications.

==> approach.tex <==
\section{Introduction}

1. Context and Importance of Automated Evaluation
   - Rapid Growth of LLMs: Highlight the emergence and proliferation of Large Language Models (LLMs) that generate high-quality, free-form text outputs across diverse domains (e.g., summarization, content creation, recommendation, profile extraction).
   - Need for Reliable Evaluation: Emphasize the importance of evaluating these outputs to ensure quality, relevance, and correctness. State that evaluation is crucial for refining models, guiding system improvements, and building trust in automated solutions.

2. Challenges in Manual Evaluation
   - Labor-Intensive and Costly: Stress that human expert evaluations are resource-intensive, both in terms of time and expense.
   - Scalability Issues: Mention how handling large datasets or complex tasks—where each output may require nuanced judgment—becomes impractical for human evaluators alone.
   - Inconsistency Risks: Human judgments can vary widely, leading to inconsistent and subjective assessments, especially when multiple experts are involved.

3. Limitations of Existing Automatic Methods
   - Algorithmic Comparisons Fall Short: Point out that while some outputs (e.g., multiple-choice answers) can be algorithmically validated against a known correct solution, many tasks (such as evaluating free-form text quality) do not lend themselves to simple automated metrics.
   - Naïve Metrics vs. Complex Outputs: Note that standard text similarity or keyword-based metrics fail to capture the nuanced attributes that experts consider (e.g., coherence, domain relevance, subtlety of interpretation).

4. Proposed Pre-Evaluation System
   - General Approach: Introduce the concept of a robust, scalable automated pre-evaluation framework that uses LLM-based pairwise comparisons and rating systems.
   - Key Idea: Explain that instead of relying on a single LLM or fixed metric, the system aggregates multiple LLM opinions and uses a rating method (like Elo) to establish a reliable ranking of outputs.
   - Versatile Application: Emphasize the universal applicability of this system, stating it can serve as a pre-evaluation layer for virtually any task where LLMs produce free-form outputs, reducing the need for large-scale human intervention.

5. Illustrative Example: Competency Profile Extraction
   - Demonstration Scenario: Present the competency profile extraction task as one illustrative application, not the sole purpose of the method.
   - Relevance of Example: Show how the pre-evaluation system can help rank competency profiles generated by multiple LLMs, ensuring that the most domain-relevant and comprehensive profiles surface.
   - Transferable Insights: Make it clear that while the paper focuses on this scenario, the underlying methodology is not tied to this domain alone.

6. Goals and Expected Outcomes
   - Primary Objective: State the goal of developing a pre-evaluation system that provides consistent, robust, and expert-correlated assessments of LLM-generated text.
   - Long-Term Vision: Indicate that such a system can significantly reduce human workload, accelerate iterative improvements in model outputs, and foster more transparent, data-driven evaluation pipelines.

7. Contributions and Significance
   - Novelty: Highlight that the approach combines multiple LLM judgments and a well-established rating framework (Elo) to address complexity and subjectivity in evaluation tasks.
   - Impact: Describe how the resulting methodology can streamline workflows in research, industry, and academia, making the evaluation of free-form text outputs more efficient and reliable.

8. Roadmap of the Paper
   - Approach Section: Will detail the methodology, including the pairwise comparison framework, bias mitigation strategies, and the Elo rating system.
   - Implementation Details: Will provide a brief overview of the technical setup and tools used.
   - Evaluation Section: Will present how the system’s results correlate with expert judgments, showcasing its capability as a pre-evaluation tool.
   - Discussion and Future Work: Will consider broader implications, limitations, and potential extensions of the approach.

\section{Background}
\todo

\section{Related Work}
\todo

\section{Approach}

\subsection{Introduction to the Proposed Methodology}

\begin{itemize}
    \item \textbf{Objective}: Present an automated evaluation strategy using Large Language Models (LLMs) to perform pairwise comparisons of items (e.g., competency profiles).
    \item \textbf{Motivation}:
    \begin{itemize}
        \item \textbf{Limitations of Human Evaluation}: High cost, time consumption, and lack of scalability for on-demand evaluations.
        \item \textbf{Challenges with Naïve LLM Evaluations}: Issues like self-consistency problems and positional biases when using LLMs directly for evaluations.
    \end{itemize}
    \item \textbf{Goal}: Develop a scalable, reliable, and automated pre-evaluation method that overcomes these challenges.
\end{itemize}

\subsection{Pairwise Comparison Framework}

\begin{itemize}
    \item \textbf{Rationale}:
    \begin{itemize}
        \item \textbf{Precision and Consistency}: Pairwise comparisons reduce subjective scaling issues inherent in scoring methods.
        \item \textbf{Relative Assessment}: Focusing on relative preferences enhances evaluation granularity and reliability.
    \end{itemize}
    \item \textbf{Framework Description}:
    \begin{itemize}
        \item \textbf{Item Pairing}:
        \begin{itemize}
            \item Every item (competency profile) is compared with every other item.
            \item For \( n \) items, there are \( \frac{n \times (n - 1)}{2} \) pairwise comparisons.
        \end{itemize}
        \item \textbf{Bidirectional Evaluations}:
        \begin{itemize}
            \item Each pair is evaluated in both possible orders (Item A vs. Item B and Item B vs. Item A) to mitigate positional bias.
        \end{itemize}
        \item \textbf{Use of Multiple LLMs}:
        \begin{itemize}
            \item Multiple state-of-the-art LLMs are employed to perform each evaluation.
            \item This results in a total of \( n \times (n - 1) \times \text{num\_LLMs} \) evaluations.
        \end{itemize}
    \end{itemize}
    \item \textbf{Evaluation Criteria}:
    \begin{itemize}
        \item LLMs assess which item better reflects specified criteria based solely on the content provided.
        \item Evaluations are designed to be objective and consistent across models.
    \end{itemize}
\end{itemize}

\subsection{Mitigation of LLM Biases}

\begin{itemize}
    \item \textbf{Prompt Design}:
    \begin{itemize}
        \item \textbf{Neutral Language}: Prompts are carefully crafted to avoid leading language and minimize biases.
        \item \textbf{Consistency}: The same prompts are used across all evaluations to ensure uniformity.
    \end{itemize}
    \item \textbf{Bidirectional Evaluations}:
    \begin{itemize}
        \item Evaluating each pair in both orders helps to counteract any positional biases inherent in LLMs.
    \end{itemize}
    \item \textbf{Retrieval-Augmented Generation (RAG) with Vector Database}:
    \begin{itemize}
        \item \textbf{Purpose}: Provide relevant examples of extractions and pairwise comparisons to ground LLM responses.
        \item \textbf{Implementation}:
        \begin{itemize}
            \item A vector database (ChromaDB) is used to retrieve similar examples.
            \item Examples are incorporated into prompts to enhance understanding and reduce biases.
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Handling Multiple Evaluations and Agreement Thresholds}

\begin{itemize}
    \item \textbf{Challenges Addressed}:
    \begin{itemize}
        \item \textbf{Self-Consistency Problems}: Variations in LLM outputs due to differences in reasoning or interpretation.
    \end{itemize}
    \item \textbf{Agreement Thresholds Analyzed}:
    \begin{itemize}
        \item \textbf{Unanimity (100\% Agreement)}: All LLMs agree on the preferred item.
        \item \textbf{90\% Agreement}: At least 90\% of LLMs agree.
        \item \textbf{75\% Agreement}: At least 75\% of LLMs agree.
        \item \textbf{50\% Agreement}: A simple majority of LLMs agree.
        \item \textbf{Individual Evaluations}: Each LLM's evaluation is considered individually without requiring agreement.
    \end{itemize}
    \item \textbf{Decision Mechanism}:
    \begin{itemize}
        \item \textbf{Outcome Determination}:
        \begin{itemize}
            \item \textbf{Win}: If the agreement threshold is met, the preferred item records a win.
            \item \textbf{Loss}: The non-preferred item records a loss.
            \item \textbf{Draw}: If the agreement threshold is not met, the outcome is considered a draw.
        \end{itemize}
    \end{itemize}
    \item \textbf{Impact on Evaluation}:
    \begin{itemize}
        \item \textbf{Higher Thresholds}: Increase confidence but may result in more draws.
        \item \textbf{Lower Thresholds}: Allow more evaluations to influence the outcome but may introduce inconsistencies.
    \end{itemize}
\end{itemize}

\subsection{Elo Rating System for Ranking Items}

\begin{itemize}
    \item \textbf{Justification}:
    \begin{itemize}
        \item \textbf{Dynamic Ranking}: Elo ratings provide a method to update item rankings based on pairwise comparison outcomes dynamically.
        \item \textbf{Standardization}: Using a well-established system ensures reliability and comparability.
    \end{itemize}
    \item \textbf{Implementation Details}:
    \begin{itemize}
        \item \textbf{Initial Ratings}: All items start with an initial rating of 1000 points.
        \item \textbf{Standard Elo Formula}:
        \begin{itemize}
            \item \textbf{Expected Score}:
            \[
            E = \frac{1}{1 + 10^{(\text{Rating}_{\text{opponent}} - \text{Rating}_{\text{player}})/400}}
            \]
            \item \textbf{Rating Adjustment}:
            \[
            \text{New Rating} = \text{Current Rating} + K \times (\text{Score} - E)
            \]
            \item \textbf{K-Factor}: Set to 32, determining the magnitude of rating changes per comparison.
        \end{itemize}
        \item \textbf{Outcome Scoring}:
        \begin{itemize}
            \item \textbf{Win}: Score = 1.0
            \item \textbf{Loss}: Score = 0.0
            \item \textbf{Draw}: Score = 0.5
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Visual Representation}

\begin{itemize}
    \item \textbf{Diagrams and Workflows}:
    \begin{itemize}
        \item \textbf{Flowchart of the Evaluation Process}:
        \begin{itemize}
            \item Illustrate the flow from profile generation, pairwise comparisons, LLM evaluations, agreement threshold application, to Elo rating updates.
        \end{itemize}
        \item \textbf{Example Diagram}:
        \begin{itemize}
            \item Show profiles passing through multiple LLMs in pairwise matchings.
            \item Visualization of Elo rating adjustments leading to a sorted list.
        \end{itemize}
    \end{itemize}
    \item \textbf{Purpose of Visual Aids}:
    \begin{itemize}
        \item Enhance understanding of the methodology.
        \item Provide clear, step-by-step representation of the process.
    \end{itemize}
\end{itemize}

\subsection{Justification of Methods and Techniques}

\begin{itemize}
    \item \textbf{Selection of LLMs}:
    \begin{itemize}
        \item Chosen for their representation of state-of-the-art capabilities.
        \item Diversity of models helps mitigate individual biases.
    \end{itemize}
    \item \textbf{Pairwise Comparisons and Elo Ratings}:
    \begin{itemize}
        \item Provide a robust framework for ranking without subjective scoring scales.
    \end{itemize}
    \item \textbf{Agreement Threshold Analysis}:
    \begin{itemize}
        \item Allows exploration of the impact of consensus levels on evaluation outcomes.
    \end{itemize}
\end{itemize}






\section{Implementation}

\subsection{Technical Details}

\begin{itemize}
    \item \textbf{Programming Languages and Tools}:
    \begin{itemize}
        \item \textbf{Python}: Used for all implementations.
        \item \textbf{APIs and Libraries}:
        \begin{itemize}
            \item \textbf{Flask}: For the web interface and expert evaluation setup.
            \item \textbf{Requests}: For sending HTTP requests to LLM APIs.
            \item \textbf{ChromaDB}: Used as the vector database for Retrieval-Augmented Generation (RAG).
            \item \textbf{NumPy and SciPy}: For statistical calculations (e.g., Spearman's rho, Kendall's tau).
        \end{itemize}
    \end{itemize}
    \item \textbf{LLMs Employed}:
    \begin{itemize}
        \item \textbf{State-of-the-Art Models}:
        \begin{itemize}
            \item 'gemma2-9b-it'
            \item 'llama-3.1-70b-versatile'
            \item 'llama-3.3-70b-versatile'
            \item 'mixtral-8x7b-32768'
            \item 'llama-3.1-8b-instant'
            \item 'llama-3.2-1b-preview'
            \item 'llama-3.2-90b-text-preview'
            \item 'gpt-4o'
            \item 'gpt-4o-mini'
        \end{itemize}
        \item \textbf{Access Methods}: Models accessed via APIs from providers like GROQ and OpenAI.
    \end{itemize}
    \item \textbf{Data Sources}:
    \begin{itemize}
        \item \textbf{Abstracts and Profiles}:
        \begin{itemize}
            \item Abstracts collected from the KIT Open Library and OpenAlex database.
            \item No preprocessing performed on the data.
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Experimental Setup}

\begin{itemize}
    \item \textbf{Profile Generation}:
    \begin{itemize}
        \item \textbf{Process}:
        \begin{itemize}
            \item Experts selected 5-10 of their own papers.
            \item Abstracts from these papers were used as input for profile generation.
        \end{itemize}
        \item \textbf{LLM Processing}:
        \begin{itemize}
            \item Each LLM generated profiles based on the provided abstracts using a standardized extraction prompt.
        \end{itemize}
    \end{itemize}
    \item \textbf{Expert Evaluation Setup}:
    \begin{itemize}
        \item \textbf{Web Interface}:
        \begin{itemize}
            \item Custom-built Flask application for experts to select papers and review generated profiles.
        \end{itemize}
        \item \textbf{Data Collection}:
        \begin{itemize}
            \item Profiles collected and stored for subsequent evaluation.
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Challenges and Solutions}

\begin{itemize}
    \item \textbf{Minimal Challenges}:
    \begin{itemize}
        \item The implementation was straightforward due to the use of established tools and APIs.
    \end{itemize}
    \item \textbf{Scalability}:
    \begin{itemize}
        \item \textbf{Solution}: Efficient handling of API requests and data storage to manage multiple evaluations.
    \end{itemize}
\end{itemize}

\subsection{Implementation Summary}

\begin{itemize}
    \item \textbf{Overall Approach}:
    \begin{itemize}
        \item Leveraged existing technologies to implement the proposed methodology efficiently.
    \end{itemize}
    \item \textbf{Focus on Methodology Over Technical Complexity}:
    \begin{itemize}
        \item Emphasis placed on developing a robust evaluation strategy rather than on complex technical implementations.
    \end{itemize}
\end{itemize}

\section{Evaluation}

\subsection{Evaluation Overview}

\begin{itemize}
    \item \textbf{Purpose}:
    \begin{itemize}
        \item To assess how well the automated evaluation (Elo rating-based ranking) matches human expert judgments in assessing the quality of competency profiles.
    \end{itemize}
    \item \textbf{Scope}:
    \begin{itemize}
        \item Comparison between the rankings produced by the automated system and those provided by human experts.
    \end{itemize}
    \item \textbf{Limitations}:
    \begin{itemize}
        \item \textbf{Incomplete Data}: The evaluation is ongoing, with participant recruitment in progress.
        \item \textbf{Sample Size}: Final results pending based on the number of experts participating.
    \end{itemize}
\end{itemize}

\subsection{Outline of the Evaluation Process}

\begin{itemize}
    \item \textbf{Expert Participation}:
    \begin{itemize}
        \item \textbf{Recruitment}:
        \begin{itemize}
            \item Experts (e.g., professors at KIT) are invited to participate via email.
        \end{itemize}
        \item \textbf{Task}:
        \begin{itemize}
            \item Experts select 5-10 of their own papers using the web interface.
            \item They are presented with generated profiles and asked to rank them based on how well they match their actual competencies.
        \end{itemize}
    \end{itemize}
    \item \textbf{Automated Evaluation}:
    \begin{itemize}
        \item \textbf{Process}:
        \begin{itemize}
            \item Profiles are ranked using the Elo rating system based on LLM evaluations.
        \end{itemize}
        \item \textbf{Comparison}:
        \begin{itemize}
            \item The automated rankings are compared to the expert-provided rankings using statistical metrics.
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Evaluation Strategy}

\begin{itemize}
    \item \textbf{Experimental Setup}:
    \begin{itemize}
        \item \textbf{Data Collection from Experts}:
        \begin{itemize}
            \item Experts select papers and review generated profiles via the web interface.
        \end{itemize}
        \item \textbf{Profile Pairing and Evaluation}:
        \begin{itemize}
            \item \textbf{Pairwise Comparisons}:
            \begin{itemize}
                \item All possible pairs of profiles are compared.
                \item For 8 profiles, \( \frac{8 \times 7}{2} = 28 \) unique pairs.
            \end{itemize}
            \item \textbf{LLM Evaluations}:
            \begin{itemize}
                \item Each pair is evaluated in both orders by multiple LLMs.
                \item Total evaluations per author: \( 28 \text{ pairs} \times 2 \text{ orders} \times 8 \text{ LLMs} = 448 \) evaluations.
            \end{itemize}
        \end{itemize}
        \item \textbf{Agreement Threshold Application}:
        \begin{itemize}
            \item Different thresholds are applied to determine outcomes for Elo rating adjustments.
        \end{itemize}
    \end{itemize}
    \item \textbf{Addressing Research Questions}:
    \begin{itemize}
        \item \textbf{Primary Research Question}:
        \begin{itemize}
            \item How effectively can an automated evaluation strategy using LLMs and an Elo rating system replicate human expert judgments in ranking competency profiles?
        \end{itemize}
        \item \textbf{Evaluation Objectives}:
        \begin{itemize}
            \item Assess the correlation between automated rankings and expert rankings.
            \item Determine the impact of different agreement thresholds on evaluation accuracy.
        \end{itemize}
    \end{itemize}
    \item \textbf{Absence of Baselines and Benchmarks}:
    \begin{itemize}
        \item \textbf{Justification}:
        \begin{itemize}
            \item The focus is on comparing the automated method directly with expert judgments.
            \item No existing baseline methods are directly comparable for this specific task.
        \end{itemize}
    \end{itemize}
    \item \textbf{Strategy Summary}:
    \begin{itemize}
        \item The evaluation strategy is designed to directly address the research question by comparing automated and expert rankings using appropriate statistical measures.
    \end{itemize}
\end{itemize}


\todo{
    Evaluation Results
}


\todo{Limitations, References, Ethicals outside of 8 Page limit but must be included}

\section{Limitations}

\begin{itemize}
    \item Compute requirements - hundreds of evaluations per profile set
\end{itemize}

\todo{Reference HoReKA}

\todo{Ethicals}
